Why Does Propositional Quantification Make Modal and Temporal Logics on Trees Robustly Hard?

Adding propositional quantification to the modal logics K, T or S4 is known to lead to undecidability but CTL with propositional quantification under the tree semantics (tQCTL) admits a non-elementary Tower-complete satisfiability problem. We investigate the complexity of strict fragments of tQCTL as well as of the modal logic K with propositional quantification under the tree semantics. More specifically, we show that tQCTL restricted to the temporal operator EX is already Tower-hard, which is unexpected as EX can only enforce local properties. When tQCTL restricted to EX is interpreted on N-bounded trees for some N >= 2, we prove that the satisfiability problem is AExpPol-complete; AExpPol-hardness is established by reduction from a recently introduced tiling problem, instrumental for studying the model-checking problem for interval temporal logics. As consequences of our proof method, we prove Tower-hardness of tQCTL restricted to EF or to EXEF and of the well-known modal logics such as K, KD, GL, K4 and S4 with propositional quantification under a semantics based on classes of trees.

==> sections/abstract.tex <==
\begin{abstract}
Adding propositional quantification to the modal logics \K, $\mathsf{T}$ or 
\Sfour is known to lead to undecidability  
%% whereas 
but \CTL with propositional 
quantification under the tree semantics 
%% (written \tQCTL{}) 
(\tQCTL{})
admits a non-elementary 
\tower-complete satisfiability problem. We investigate the complexity of strict 
fragments of \tQCTL{} as well as of the modal logic \K with propositional 
quantification under the tree semantics. More specifically, we show that \tQCTL{} 
restricted to the temporal operator~$\EX$ is already \tower-hard, which is 
unexpected as
%% , for instance, 
$\EX$ can only enforce local properties. 
When \tQCTL{} restricted to $\EX$ is interpreted on $N$-bounded trees for 
some~$N \geq 2$, we prove that the satisfiability problem is \aexppol-complete; 
\aexppol-hardness is established by reduction from a recently introduced
tiling problem, instrumental for studying the model-checking problem for 
interval temporal logics. As 
%% significant 
consequences of our proof method, 
we prove \tower-hardness of \tQCTL{} restricted to  $\EF$ or to $\EX\EF$ and  
of the well-known modal logics \K, \KD, \GL, \Sfour, \Kfour and 
\Dfour, with propositional quantification under a semantics based on  classes of trees. 
%% under a semantics for appropriate  classes of trees. 
\end{abstract}
